$C^3$: Compositional Counterfactual Contrastive Learning for Video-grounded Dialogues

Video-grounded dialogue systems aim to integrate video understanding and dialogue understanding to generate responses that are relevant to both the dialogue and video context. Most existing approaches employ deep learning models and have achieved remarkable performance, given the relatively small datasets available. However, the results are partly accomplished by exploiting biases in the datasets rather than developing multimodal reasoning, resulting in limited generalization. In this paper, we propose a novel approach of Compositional Counterfactual Contrastive Learning ($C^3$) to develop contrastive training between factual and counterfactual samples in video-grounded dialogues. Specifically, we design factual/counterfactual sampling based on the temporal steps in videos and tokens in dialogues and propose contrastive loss functions that exploit object-level or action-level variance. Different from prior approaches, we focus on contrastive hidden state representations among compositional output tokens to optimize the representation space in a generation setting. We achieved promising performance gains on the Audio-Visual Scene-Aware Dialogues (AVSD) benchmark and showed the benefits of our approach in grounding video and dialogue context.

==> table/additional_result.tex <==
\begin{table*}[htbp]
\centering
\small
\begin{tabular}{lcccccc}
\hline
          & d   & h & B-4   & M     & R     & C     \\
          \hline
MTN       & 128 & 8 & 0.376$\pm0.003$ & 0.253$\pm0.001$ & 0.534$\pm0.003$ & 0.996$\pm0.007$ \\
\hline
MTN+$C^3(\mathcal{I}^{+/-})$ & 128 & 8 & 0.398$\pm0.003$ & 0.262$\pm0.001$ & 0.549$\pm0.002$ & 1.040$\pm0.003$ \\
MTN+$C^3(\mathcal{I}^{+/-})$ & 64  & 8 & 0.370$\pm0.002$ & 0.250$\pm0.002$ & 0.530$\pm0.001$ & 0.940$\pm0.004$ \\
MTN+$C^3(\mathcal{I}^{+/-})$ & 128 & 1 & 0.352$\pm0.004$ & 0.242$\pm0.002$ & 0.521$\pm0.002$ & 0.917$\pm0.003$ \\
MTN+$C^3(\mathcal{I}^{+/-})$ & 128 & 2 & 0.389$\pm0.003$ & 0.253$\pm0.001$ & 0.536$\pm0.003$ & 1.018$\pm0.006$ \\
MTN+$C^3(\mathcal{I}^{+/-})$ & 128 & 4 & 0.393$\pm0.002$ & 0.259$\pm0.001$ & 0.545$\pm0.002$ & 1.028$\pm0.007$ \\
\hline
MTN+$C^3(\mathcal{H}^{+/-})$ & 128 & 8 & 0.393$\pm0.003$                     & 0.260$\pm0.003$                     & 0.545$\pm0.001$                     & 1.029 $\pm0.005$                    \\
MTN+$C^3(\mathcal{H}^{+/-})$ & 64  & 8 & 0.372$\pm0.002$                     & 0.248$\pm0.001$                     & 0.527$\pm0.002$                     & 0.937$\pm0.006$                     \\
MTN+$C^3(\mathcal{H}^{+/-})$ & 128 & 1 & 0.351$\pm0.003$                     & 0.232$\pm0.002$                     & 0.503$\pm0.004$                     & 0.882$\pm0.008$                     \\
MTN+$C^3(\mathcal{H}^{+/-})$ & 128 & 2 & 0.386$\pm0.005$                     & 0.251$\pm0.004$                     & 0.534$\pm0.001$                     & 1.000 $\pm0.009$                    \\
MTN+$C^3(\mathcal{H}^{+/-})$ & 128 & 4 & 0.391 $\pm0.002$                    & 0.257$\pm0.001$                     & 0.543$\pm0.001$                     & 1.019$\pm0.005$ \\
\hline
\end{tabular}
\caption{
Additional experiment results with standard deviations on 4 metrics: B-4 (BLEU-4), M (METEOR), R (ROUGE-L), and C(CIDEr). $d$ denotes the embedding dimension and $h$ denotes the number of attention heads.
}
\label{tab:additional_results}
\end{table*}
